Purely Bayesian counterfactuals versus Newcomb's paradox

This paper proposes a careful separation between an entity's epistemic system and their decision system. Crucially, Bayesian counterfactuals are estimated by the epistemic system; not by the decision system. Based on this remark, I prove the existence of Newcomb-like problems for which an epistemic system necessarily expects the entity to make a counterfactually bad decision. I then address (a slight generalization of) Newcomb's paradox. I solve the specific case where the player believes that the predictor applies Bayes rule with a supset of all the data available to the player. I prove that the counterfactual optimality of the 1-Box strategy depends on the player's prior on the predictor's additional data. If these additional data are not expected to reduce sufficiently the predictor's uncertainty on the player's decision, then the player's epistemic system will counterfactually prefer to 2-Box. But if the predictor's data is believed to make them quasi-omniscient, then 1-Box will be counterfactually preferred. Implications of the analysis are then discussed. More generally, I argue that, to better understand or design an entity, it is useful to clearly separate the entity's epistemic, decision, but also data collection, reward and maintenance systems, whether the entity is human, algorithmic or institutional.

==> proof_impossibility.tex <==
\subsubsection{Proof of impossibility}
\label{sec:proof_impossibility}

We now have all the necessary ingredients to prove Theorem \ref{th:impossibility}.

\begin{proof}[Proof of Theorem \ref{th:impossibility}]
  Call \textsc{X} and \textsc{Y} the two decisions available to \dan{}. We suppose that \OM{} that has access to sufficiently many data $D_\Omega$ to be $\delta$-omniscient about \dan{}'s decision (with $0 < \delta < \varepsilon < 1/2$), and to know more than \emma{}. \OM{} now makes the prediction $\omega \triangleq \pb{\textsc{X} \st D_\Omega}$ about \dan{}'s decision.
  If $\omega \geq 1/2$, then \OM{} then gives \alice{} no reward ($\mathcal R=0$). Otherwise, if $\omega < 1/2$, then \OM{} gives \alice{} the reward $\mathcal R=1$. Using the law of total probability, we then have
  \begin{align}
    &\expect{\mathcal R \st D_{\bf E} \wedge \textsc{X}}
    % = \expectVariable{\omega}{\expect{\mathcal R \st D_{\bf E} \wedge \textsc{X} \wedge \omega} \st D_{\bf E} \wedge \textsc{X}} \\
    = \sum_{\omega} \expect{\mathcal R \st D_{\bf E} \wedge \textsc{X} \wedge \omega} \pb{\omega \st D_{\bf E} \wedge \textsc{X}} \\
    &\qquad = \pb{\omega = \delta \st D_{\bf E} \wedge \textsc{X}}
    = \frac{\pb{\textsc{X} \st \omega = \delta \wedge D_{\bf E}} \pb{\omega=\delta \st D_{\bf E}}}{\pb{\textsc{X} \st D_{\bf E}}}.
    % \\
    % &\qquad = \frac{\delta (1-\sfrac{\varepsilon}{2}+O(\delta))}{1-\sfrac{\varepsilon}{2}} \rightarrow 0.
  \end{align}
  Note that by the authority theorem \ref{th:authority}, since \OM{} knows more than \emma{}, we have $\pb{\textsc{X} \st \omega = \delta \wedge D_{\bf E}} = \delta$.
  Moreover, denoting $p \triangleq \pb{\omega = 1-\delta \st D_{\bf E}}$ \emma{}'s prior on \OM{} predicting \textsc{X}, and $q= \pb{\textsc{X} \st D_{\bf E}}$ \emma{}'s prior on \dan{} deciding \textsc{X},
  by Lemma \ref{lemma:quasi_omniscience}, we have $q=\delta + (1-2\delta) p$.
  This then yields $p = \frac{q-\delta}{1-2\delta}$, and $1-p = \frac{1-\delta-q}{1-2\delta}$. As a result,
  \begin{equation}
    \expect{\mathcal R \st D_{\bf E} \wedge \textsc{X}} = \frac{\delta (1-\delta-q)}{q(1-2\delta)} \rightarrow 0,
  \end{equation}
  in the limit $\delta \rightarrow 0$.
  Similarly, we have
  \begin{align}
    \expect{\mathcal R \st D_{\bf E} \wedge \textsc{Y}}
    &= \frac{\pb{\textsc{Y} \st \omega = \delta \wedge D_{\bf E}} \pb{\omega=\delta \st D_{\bf E}}}{\pb{\textsc{Y} \st D_{\bf E}}} \\
    &= \frac{(1-\delta)(1-q-\delta)}{(1-2\delta)(1-q)} \rightarrow 1.
  \end{align}
  Thus for $\delta$ small enough, we see that, by deciding \textsc{X}, \dan{} made the counterfactually wrong decision.
\end{proof}

